High Performance Zero-Memory Overhead Direct Convolutions

The computation of convolution layers in deep neural networks typically rely on high performance routines that trade space for time by using additional memory (either for packing purposes or required as part of the algorithm) to improve performance. The problems with such an approach are two-fold. First, these routines incur additional memory overhead which reduces the overall size of the network that can fit on embedded devices with limited memory capacity. Second, these high performance routines were not optimized for performing convolution, which means that the performance obtained is usually less than conventionally expected. In this paper, we demonstrate that direct convolution, when implemented correctly, eliminates all memory overhead, and yields performance that is between 10% to 400% times better than existing high performance implementations of convolution layers on conventional and embedded CPU architectures. We also show that a high performance direct convolution exhibits better scaling performance, i.e. suffers less performance drop, when increasing the number of threads.

==> 030method.tex <==
\subsection{Convolution overview}
The CNN forward process is to apply a filter on the image data, convolve, and generate the output. Picture

The plain CNN forward process is shown in list \ref{CNNcode}
% \begin{algorithm}%[htb]
%   \footnotesize
%   \caption{\label{alg:conv} Convolution forward pass}
%   \begin{tabular}{@{}lll@{}}
%       {\bf Input} 
%     & $G(\V, \E, \Adj )$~~~~~graph \\

%       {\bf Input} 
%     & $G(\V, \E, \Adj )$~~~~~graph \\

    
%   \addlinespace[0.5mm]
% %    \multicolumn{3}{l}{~~~end} \\
%     \multicolumn{3}{l}{~~~{\bf return} $\W$} \\  
%     \addlinespace[1mm]
%   \end{tabular}
% \end{algorithm}

\begin{lstlisting}[language=C, frame=single, float, breaklines=true,  caption={CNN forward process}, label=CNNcode]  % Start your code-block

//iteration along input channel
for (ich=0; ich<InCh; ich++)
//iteration along output channel
  for (och=0; och<OuCh; och++)
  //iteration along output row
    for (or=0; or<OuR; or++)
    //iteration along output col
      for (ol=0; ol<OuL; ol++)
      //iteration along fil row
        for (fr=0; fr<FilR; fr++)
        //iteration along fil col
          for (fl=0; fl<FilL; fl++)
Output[och][or][ol] += Input[ich][or*stride+fr][ol*stride+fl] * Fils[ich][och][fr][fl];
    
\end{lstlisting}

\renewcommand{\arraystretch}{1.2}
\begin{table}
  \begin{tabular}{ l | p{5cm} }
    \hline
     \N & The input channel size\\ 
     \Ch & The output channel size\\ 
     \Bat & The batch size\\
     \Ho, \Hi, \Hf & The height of output, input, filter\\ 
     \Wo, \Wi, \Wf & The width of output, input, filter\\
     \Hob, \Hib, \Hfb & The block size of the output, input, filter height\\
     \Wob, \Wib, \Wfb & The block size of the output, input, filter width\\
     \hline
     $\ci$, $\co$, $\cb$ & iterator along input channel, output channel, batch dimension \\
     \wo, \wi, \wf & iterator along output, input, filter width dimension \\
     \ho, \hi, \hf & iterator along output, input, filter height dimension\\
     \hline
  \end{tabular}
  \caption{Notation } 
  \label{table:notation}
\end{table}


It consists of six loops. Two loops (ich, och) correspond to the image channels (input channels and output channels). Two loops(or, ol) correspond to the output image (output row and output column respectively). Two loops (fr, fl) correspond to the filter sizes). 

\subsection{Motivation: MM lessons}
IMPORTANT: can you dig into the matrix paper to find out why they break their loops that way? Then you can find answers on how to explain your methods.

\subsection{Forward process}
In this section, we first present how the forward process works. We will explain the designs on SIMD, cache locality, data layout,.

There are two key points related with optimizing convolution performance: cache locality and data layout. 

In the matrix multiplication example, these two points are the essential to obtain the high performance. If we are to get peak performance out of convolution, the same analysis routines could be applied. In the MM case, the program consist of three loops, but in the optimized version, the program is eventually blocked into six loops Fig~\ref{}. The blocking on the M, N dimensions divides the multiplicand and multiplier matrixes A and B into small tiles, because . Then on top of that, the loops are further divided because one wants to leverage the SIMD registers. 

And MM can also adopt to inverse case, because it allows data reshape between loops.

Convolution could adopt the similar stratege, but it is much difficult because it has more loops, which means more design space than the two-dimensional matrix multiplication. 


\textbf{SIMD}
In order to do SIMD, the channel should be the fastest dimension.
It has been realized by many work that the channel dimension should be the fastest changing dimension, because 1). There are parallelism along the channel dimension, 2). It is more regular to (SIMD) parallelism along the channel dimension. 

On the other hand, there are also parallelism along the image row and column dimensions.  Every micro-block of input image matrixes has to multiply with the filter matrixes and reduce to one element of output matrixes. Therefore, 

\textbf{register blocking}
Why choose reuse output matrixes and not input matrixes? 
kernel size choice
outer product

\textbf{blocking}
Because the dimension is too long, blocking helps reuse. We need block at the input and output channel dimensions, and the output image width and height dimensions. 
To design the optimal blocking scheme, the loop order matters because it determines which data to be reused. 

option 1: Input matrix and filter matrixes can be reused. 
option 2: 

\textbf{loop order to maximize reuse}
The INNER loop around macro kernel: it can reuse the filter matrixes for Nr times.
the subsequent outer loop is output dimension: because then it can reuse the filter matrixes
the subsequent outer loop is output channel: because then it can reuse the input matrixes.
The next subsequent outer loop is input channel: because then it can reuse 


\textbf{data layout choices for forward process}
Given those parameters, the data layout should align with those parameters.
The filter data should be [InCh/INNER][OuCh/Mr][Inner][FS][FS][Mr] or [InCh/Inner][OuCh/Mr][FS][FS][INNER][Mr]. The second requires the macro kernel loop to loop around the INNER first then the filter dimension next.
Picture illustrates how the used data change as the loop dimensions

Image data should be [Ich/Mr][IS][IS][Mr]. The Mr is at the lowest dimension because it is the vectorization dimension. But contrary to what most people think, it is not all the way to the entire dimension. Because the micro-kernel iterates along the image size dimensions first. If . But the image layout could also be [Ich/(Mr*INNER)][IS][IS][Mr*INNER] then it requires the microkernel to iterate along the INNER first then the image dimensions. And then the correspondingly 



\textbf{parametrize and adapt to different architectures}
There are three parameters in total. two parameters are related with cache blocking, determining the data layout: Input image block, FilSize block. Two parameters are related with register blocking:. 

Mr, Nr is the register blocking parameter, they are determined by the CPU registers;
INNER is the parameter associated with the micro-kernel: it is related with amortize overheads


Mr*FS*FS*INNER is the iterations that the output registers been reused. So Mr*INNER should be large to amortize the register access (maximize the register reuse), but they shouldn't go beyond the L1 cache size. 

We empirically enumerate the possible parameters and the choose out the best one.


\subsection{Optimal Data layout for forward, backward process codesign}
\textbf{brief overview about backward image process and backward filter process}

\textbf{SIMD parallelism for Backward image process}
The inner-most parallelism for backward image process is very similar to forward process, which leverages the parallelism along the channel dimension and the image row/col dimensions. 

\textbf{SIMD parallelsim for backward filter process}
The inner-most parallelism for backward image process leverages the parallelism along the output row/col dimensions. 

List showing the different blocking parameters, forward and backward get different performance tradeoffs: The larger blocking parameter benefits the forward process, however harms the backward.



\subsection{Multi-threading} 
The loop to parallize is the Och dimension. So each thread will compute part of the output matrixes.

\textbf{Different sizes}
1st layer has different performance than the rest layers. Because it is the input of image. RGB usually has three channels. 
One way to optimize is to utilize the fact that there are multiple batches and parallelize across batch dimension. Then this kind of computation can utilize .... But in the infering process, there is usually only 1 image. (List of OpenBLAS and MKL will get worse performance in the first layer)

\subsection{Wrap up}



==> compatibility.tex <==

\subsection{Changes to other layers in the network}

\subsubsection{Activation and Skip Layers}
Activation layers such as ReLU and skip layers found in ResNets are
essentially element-wise operations. These require no change to
existing algorithm in terms of correctness. 

\subsubsection{Subsampling Layer}
Other commonly used layers such as max-pooling 


==> data_layout.tex <==

\subsection{Data layout} 



Secondly, for a convolution neural network, besides the input data layer and the output data layers, all the layers in-between are hidden. In other words, a high level programmer who uses a CNN module does not need care about those middle layers details. This grants us the freedom to alter the data layout between layers as long as the layout and computation is consistent.

The shortages of those work are: They only consider a small set of layout choices among all the layout possibilities. Their parallelism relies on the Batch dimension. Their layout choice is not consistent between layer, therefore they require layout transforming between layers, which brings extra overheads. Moreover, none of those work considers for backward propagation process. The optimal layout for forward process may turn out to be not suitable for backward propagation.    

In this section, we note the optimal data layout can be determined based on the computing strategy. The principles are as follows:

It is without doubt that the layout of the data is essential to performance. A good data layout gives two-fold benefits: 1). putting data that are accessed consecutively together can benefit from streaming access. 2). The fast-changing dimension decides if one can utilize SIMD operation parallelism or not.

\subsubsection{Feature map data layout} 
We need design the layout for both feature map data and filter data. Let's first consider the layout choice for feature map data. 
The feature map is a 3D data volume. We use $W$ $H$ $C$ to represent the width, height, and channel dimensions of these data volume. Therefore, there are at least six layout ways by exhausting the factorial possibilities. 

Firstly, based on the micro-kernel access pattern, the choice narrows down to those with $C$ as the fastest-changing dimension. 

There are several facts affecting the feature map data layout:
Firstly, the SIMD instruction has to load data from consecutive memory
Secondly, it is expensive to load SIMD from unaligned memory region

Their layout is related with our blocking scheme mentioned in previous section. As we mentioned in the previous section that the micro-CNN performs updating in registers as outer product. Therefore, to exploit the SIMD instructions, either channel dimension $\Ci$ or size dimension should be the fastest changing dimension. And if we choose the size dimension as the fastest changing dimension, it will result in unaligned memory access to the memory because the consecutive iterations accesses overlapping regions of \OU as shown in Fig .

Then, the next changing dimension could be either $W$ or $H$ depending on the iterates is row or column first. But since most of the image has the same column and row size, therefore it does not have a big difference.

Next, we show that the $WHC$ is not the optimal layout. The $WHC$ data layout results in inconsecutive memory access.
Therefore, the final layout for feature map is N16HWn.

\subsubsection{filter data layout}
Now we have made the choice the feature map. Next, let's discuss the layout for filter data. The filter data is a data volume of four dimensions: $W$ $H$ $Ci$ $Co$.

\textbf{the side benefit} this layout gives is that....

%It is important to do packing. Packing brings remote data close in cache. Data will have better locality when they are allocated far apart. Normally, two packing routines should be inserted in the CNN computation: one routine packs the IMG data, and the other packs FIL data.\\
%\textbf{WHNC}\\
%\textbf{NCWH}\\
%\textbf{CNWH}\\
%\textbf{CbNbWHcn}\\

